Any-resolution Training for High-resolution Image Synthesis

Generative models operate at fixed resolution, even though natural images come in a variety of sizes. As high-resolution details are downsampled away and low-resolution images are discarded altogether, precious supervision is lost. We argue that every pixel matters and create datasets with variable-size images, collected at their native resolutions. To take advantage of varied-size data, we introduce continuous-scale training, a process that samples patches at random scales to train a new generator with variable output resolutions. First, conditioning the generator on a target scale allows us to generate higher resolution images than previously possible, without adding layers to the model. Second, by conditioning on continuous coordinates, we can sample patches that still obey a consistent global layout, which also allows for scalable training at higher resolutions. Controlled FFHQ experiments show that our method can take advantage of multi-resolution training data better than discrete multi-scale approaches, achieving better FID scores and cleaner high-frequency details. We also train on other natural image domains including churches, mountains, and birds, and demonstrate arbitrary scale synthesis with both coherent global layouts and realistic local details, going beyond 2K resolution in our experiments. Our project page is available at: https://chail.github.io/anyres-gan/.

==> sections/sm_02_experiment.tex <==

\section{Experiments}\label{sec:sm_experiments}

\subsection{Dataset Collection}

\input{tables/sm_dataset_source}

To collect our varied-size dataset, we scrape image collections from Flickr photo groups (Tab.~\ref{tab:sm_dataset_source}). In cases where a standard fixed-resolution dataset is available (\eg LSUN Churches~\cite{yu15lsun}), we seek to find photos that approximately match the domain of the standard dataset. Due to domain mismatches between LSUN and the photos scraped from Flickr, we manually filter the collected images to approximately match the LSUN domain, which remains tractable for the few thousand HR images used in the patch-based training phase. As is standard practice~\cite{thomee2016yfcc100m,park2020swapping},
and to not violate license permissions, we will release the image IDs but not the images directly.

\begin{figure}[t] %
  \begin{center}
    \includegraphics[width=0.8\textwidth]{figures/fid_vs_patchfid.pdf}
  \end{center}
  \caption{\small Preprocessing for FID and patch-FID (pFID). FID evaluates global structure, but downsamples all images to a common 299px size which ignores higher resolution details. pFID takes images crops instead rather than downsampling to capture texture realism at higher resolutions. We use both to measure structure and texture properties. \label{fig:fid_vs_patchfid}}
\end{figure}

\subsection{Patch-FID}

\begin{wrapfigure}{r}{0.35\textwidth}
    \vspace{-2mm}
  \begin{center}
    \includegraphics[width=.35\textwidth]{figures/CR_correlation.pdf}
  \end{center}
  \vspace{-4mm}
  \caption{\small pFID vs FID@1024. The metrics are largely correlated, but
  FID@1024 generates images at 1024 resolution and then downsamples images, assuming a fixed-size dataset. On other domains
  where a ground-truth HR dataset is not available, we primarily use pFID to
  measure sample quality. \label{fig:sm_correlation}}
  \vspace{-2mm}
\end{wrapfigure}

We describe details of our Patch FID metric, introduced in \lucy{Section 4.1} of the main paper. The metric is aimed at better capturing the realism of details at high resolution by avoiding downsampling to capture texture details. 
In our setting, we have a smaller number of real images present at various resolutions. Standard FID, which focuses on global structure, does not capture these varied-resolution details.
We modify the FID 
pipeline to avoid downsampling global images at higher resolutions to a fixed
299 pixel width. Instead, we randomly sample patches of size \PatchResolution from real
images at global scale \FullImageResolution and locations \Coordinates, and
generate the corresponding patch  
\Generator(\LatentCode,\Coordinates,\FullImageResolution). 
The number of samples is crucial to getting an accurate estimate in FID calculation~\cite{chong2020effectively}, and 50,000 is typically used. A benefit of this patch-sampling procedure also means that we can obtain the necessary large number of patches for FID computation, more than the available number of real images in the HR dataset.
In the Mountains
generator, where the patch size \PatchResolution is larger than 299, we
subsequently also select a random 299-pixel crop from the patches to compute the
image features. Because this avoids downsampling the generated content, we find
that it is more sensitive to image quality at high resolutions. Using the full
FFHQ dataset as ground-truth, we find that our patch-FID metric is largely
correlated to the standard FID numbers at 1024 resolution
(Fig.~\ref{fig:sm_correlation}). Therefore, we use Patch-FID as a metric of
sample quality on our datasets collected from Flickr, when a full
high-resolution dataset of images all at the same resolution is not available.





\subsection{Additional quantitative results}\label{sec:sm_results}

In \lucy{Table 3} of the main text, we report
comparisons of our method and off-the-shelf super-resolution methods using the
patch-FID metric. We report additional metrics in Table~\ref{tab:sm_SR} here,
including the FID at base resolution (the result of the pretraining step), and
FID at a higher resolution after downsampling all images in the HR dataset
(between 5k-10k images, which is lower than the typical 50k used to compute FID)
to a common size.  Notably, the base resolution FID is largely similar before
and after patch-based training, and in the case of FFHQ and Birds, patch-based
training at higher resolutions even improves the low-resolution FID. Without
direct multi-scale training, however, the fixed-size model obtained from the
pretraining step does not naturally generalize to higher resolutions. We find
that our pFID metric is more discriminative to differences in image quality at
higher resolutions. In particular, the LIIF super-resolution model tends to
obtain better FID@1024 (corresponding to super-resolving generated images to 1024 resolution and computing FID) compared to Real-ESRGAN, but the outputs are visually
blurry. Because our pFID does not perform downsampling, it can better capture
this blurriness, reflected in an increased pFID. In another variant, we compute
pFID on patches of size 1024 synthesized by the Mountain generator, and then
subsequently downsample them, which we denote as pFID~(down), rather than cropping.
Again, we find that this downsampling operation can obscure image deterioration
at higher resolution, producing artificially lower FID scores compared to pFID
computed without downsampling. 

\input{tables/sm_table_SR}


\subsection{Comparison to powers-of-two synthesis} Using the same set of
generator weights, our model can synthesize images at a specified scale
by simply providing the corresponding \FullImageResolution and \Coordinates
inputs. On the other hand, other methods for multi-resolution
synthesis~\cite{lin2021anycost,karras2017progressive,denton2015deep,karnewar2020msg}
generate images that are iteratively enlarged by a factor of two, by adding
additional network layers. These methods are typically introduced to impove
training stability. For this baseline, we modify the recent Anycost-GAN~\cite{lin2021anycost}
framework to fit our varied-size training setting. Specifically, we downsample
all images in FFHQ6K to the nearest power of two, and train the corresponding
network layers only on the appropriate subset of data. To generate at any
resolution below 1024, we take the nearest model output that is larger than the
target resolution, and apply Lanczos downsampling. Similar to our approach, we
start with a pretrained model at 256 resolution, and initialize both the
generator and discriminator with pretrained weights. Because each increase in
output resolution involves training additional weights, and the number of images
at a given resolution decreases as resolution increases, we find that this
training approach yields visual artifacts at higher resolutions, shown in
Fig.~\ref{fig:sm_anycost}. 

\begin{figure}[ht!]
\centering
\includegraphics[width=\textwidth]{figures/CR_anycost.pdf}
\caption{\label{fig:sm_anycost}\small Using the same FFHQ6K dataset, we train an Anycost-GAN~\cite{lin2021anycost} and compare it to our model. While Anycost-GAN adds additional modules to increase synthesis resolution, our model shares weights across resolutions. Note that the output from Anycost-GAN contain more visual artifacts, particularly in finely textured regions such as hair.}
\end{figure}

\subsection{Comparison to Oracle Generator}\label{sec:sm_oracle}


In \lucy{Section 4} of the paper, we describe our experimental setup on the face domain, and in \lucy{Table 5} in the paper, we show competitive performance training on few HR images, even compared training on the whole HR dataset. We provide additional details and visualizations here.

We use the FFHQ dataset as a collection of 70k high-resolution
ground-truth images. To simulate more ``in-the-wild''
settings, we use a fraction (6k) of HR images for patch-based training
with a generator of size $\PatchResolution=256$, where only 1k of the images are
the full 1024 resolution, and the remainder are uniformly downsampled between
512 and 1024 prior to training. As a comparison, we also evaluate two oracle
models that train a generator directly for the $s=1024$ global image, using the
entire 70K images in the FFHQ dataset, and Lanczos downsample the result for FID
computations at other resolutions.
We also evaluate a variant of pFID, by holding the scale \textit{fixed} at the maximal resolution and randomly sampling crop locations (pFID 1024), in addition to our original pFID metric that randomly samples both scale and location (pFID random). Note that this evaluation is only possible for FFHQ controlled setting, as all images are present at the maximal 1024 size.


\input{tables/ffhq_t5}

Despite being trained to generate patches, our generator can approximately match
the frequency content in real images, and that of a StyleGAN3 model trained for
1024 resolution generation on the full FFHQ dataset (Fig.~\ref{fig:sm_fft}).
While StyleGAN2 achieves better FID than StyleGAN3, we find that it has a
different frequency profile that is less similar to that of real images. We
compare the FID of these oracle models with our continuous patch model in
Tab.~\ref{tab:sm_oracle}. While the oracles can achieve lower FID and pFID variants, we note that
training the oracle assumes that a sufficient number of high-resolution images
of the same size are available, and trains the model specifically for a fixed
resolution, whereas we employ mixed resolution training on fewer than 10\% of
the full HR dataset. Our training strategy therefore allows us to take advantage of the
varied resolutions of images in the wild, which is not possible in the oracle setting. 

\begin{figure}[ht!]
\centering
\includegraphics[width=\textwidth]{figures/CR_fft.pdf}
\includegraphics[width=\textwidth]{figures/CR_fft_slice.pdf}
\caption{\label{fig:sm_fft}\small Comparison of frequency distribution. We plot the frequency spectrum of real images, StyleGAN2 and StyleGAN3 trained on the entire FFHQ dataset at 1024 resolution, and our Patch Generator which is trained on $\PatchResolution \times \PatchResolution$ patches of FFHQ6K (which contains approximately 1k images at 1024 resolution and 5k at lower resolutions). The frequency distributions are similar, suggesting that even a smaller generator is able to approximate fine textures well.}
\end{figure}

\subsection{Additional Model Variations}\label{sec:sm_model_variations}

In \lucy{Section 4.2} of the main text, we describe and study variations of our model. Here, we provide additional quantitative and qualitative results and study additional factors.

\input{tables/ffhq_t3}

\begin{figure}[!tbh]
\centering
\includegraphics[width=\textwidth]{figures/CR_model_variations.pdf}
\vspace{-10mm}
\caption{\small Qualitative examples of model variations. (Top) Using an inverse teacher loss and the scale conditioning branch generates sharper details while also preserving similarity to the base image. (Bottom) We compare our multi-size training approach to methods that
do not take advantage of different image sizes and instead train for a fixed resolution. Fixed-resolution training cannot generalize to other resolutions, and upsampling images leads to blurring. Our final model is able learn from mixed-resolution training images and also synthesize at arbitrary resolutions.}
\label{fig:sm_variations}
\end{figure}

\input{tables/ffhq_t2}
\myparagraph{Alternative metrics}
In addition to FID and pFID, we also report precision and recall~\cite{sajjadi2018assessing} for our model, naive upsampling, and super-resolution models (Tab.~\ref{tab:sm_ffhq_addtl_metrics}). Super-resolution obtains lower precision (suggesting out-of-distribution results) and similar or lower recall. Upsampling obtains similar or better precision, but lower recall (suggesting that is does not sufficiently cover the real image distribution). Here, we also include pFID measured at the maximum resolution for FFHQ (1024).

\myparagraph{Variations on teacher regularization.} In the main text, we
introduce variations on the teacher regularization including ``forward'' and
``inverse'' loss formulations, and discarding the teacher regularization
all-together. Tab.~\ref{tab:teacher} shows the FID comparisons of these three
variants, in which the ``inverse'' loss obtains the best FID scores at the
highest 1024 resolution. Adding the scale-conditioning branch to inject scale
information throughout the generator further improves FID@1024 and pFID. We show
qualitative examples in Fig.~\ref{fig:sm_variations} (top), where the inverse teacher
with scale-conditioning input can synthesize the cleanest details while still
being similar to the base image.



As default, we set $\lambda_\text{teacher}=5$ during the patch-based training
phase. Changing $\lambda_\text{teacher}$ balances between local image quality
and similarity to the base resolution image, where higher
$\lambda_\text{teacher}$ offers the most similarity to the base resolution with
lower L1 difference, but lower $\lambda_\text{teacher}$ improves pFID,
suggesting better quality of the synthesized patches
(Tab.~\ref{tab:teacher_weight}). 

\begin{figure}[!tbh]
\centering
\includegraphics[width=\textwidth]{figures/CR_dataset_size_loss.pdf}
\caption{\small Number of training images. While FID numbers are similar, we find that using 1K HR images for training shows some evidence of divergence. The training dynamics of 5K images is similar to that of the full dataset. }
\label{fig:dataset_size}
\end{figure}

\myparagraph{Fixed-size vs Multi-size training.} Fig~\ref{fig:sm_variations} (bottom)
shows an example of a synthesized patch comparing our multi-size training to
strategies of fixed-size training. Fixed-size training does not naturally
generalize to other sizes, causing deterioration in image quality when sampled
at resolutions not equal to the training resolution. Upsampling the training
images to a common resolution introduces blurriness in the synthesized output.
The result of training on only the subset of images at 1024 resolution looks
qualitatively similar to that of multi-scale training, but multi-scale training
attains better FID metrics and is able to use more images for training.


\myparagraph{Changing the number of training images.} While the model FID scores
remain largely similar (within a range of 0.3) when training on 1k to 70k
high-resolution images, we found that using 1k images showed some evidence of
training divergence (Fig.~\ref{fig:dataset_size}). On the other hand, the
training trajectory of using 5k images looks largely similar to that of using
the full HR dataset (70k) images. Therefore, when collecting images for the
remaining domains, we aim to collect between 5k-10k images to construct the HR
dataset. 

\begin{figure}[ht!]
\centering
\includegraphics[width=\textwidth]{figures/CR_extrapolation_ffhq.pdf}
\caption{\label{fig:extrapolation}\small Impact of sampling resolutions. Using the same model architecture and FFHQ6k dataset, we sample images (top) from 256 to 512 resolution, and (bottom) from 512 to 1024 resolution. The dotted line indicates when inference resolution exceeds the maximum training resolution. Watery artifacts start to appear when extrapolation, but this can be tempered by simply training on patches from larger images.}
\end{figure}

\myparagraph{Investigating the impact of sampling resolutions.} Our FFHQ6k
dataset contains images between 512 and 1024 resolution, and during training the
images are randomly downsampled from their native resolution, and can be
optionally clipped at an upper resolution. Here, we conduct experiments to study
the effects of these sampling ranges. When training the model on resolutions
\FullImageResolution sampled between 256 and 512, the image quality declines by
1024 resolution at inference time and contains visual artifacts
(Tab.~\ref{tab:sm_extrapolation}, Fig.~\ref{fig:extrapolation}). Taking the same
image and model architecture, but instead training on resolutions between 256 and 1024
offers better FID@1024, and sampling from 512 to 1024 resolution further
improves FID@1024. As before, all models are trained on patches of size
$\PatchResolution=256$, and the model is jointly trained on the fixed-size
dataset to preserve FID@256. Accordingly for the other domains, our sampled
resolutions for HR dataset range between the native resolution
$\NativeResolution$ and the minimum resolution of the HR images. These results
suggest that the synthesized resolution can be dictated by the training images;
simply adding patches from higher resolution images can allow the same model to
better synthesize at a higher resolution.\lucy{
We also tried an experiment using a separately trained smaller 128px patch generator and the same 512 to 1024 resolution patch sampling scheme, but obtained worse FID (8.38 at 1024 resolution compared to 4.16 for our default model); we hypothesize this is because may be due to worse FID from the initial pretraining phase that carries over to the patch training phase (5.14 compared to 3.71 for our default model).}


\input{tables/ffhq_t4}

\myparagraph{Changing the discriminator.} Our final model introduces changes to the generator, but keeps the same discriminator from the initial pretraining step. During patch-training, the discriminator must also learn to distinguish between real and synthesized patches. Here, we investigate alternatives of changing the discriminator setup (Tab.~\ref{tab:sm_disc_variations}). (1) We remove sampling from the LR dataset, now causing the discriminator to focus entirely on patches. This causes pFID to improve but the remaining global FIDs to worsen. In particular, this allows the generator to forget how to synthesize at the base resolution, causing a large increase in FID@256. The impact of sampling from the base resolution and the teacher regularization have similar outcomes: both encourage global coherence, but the teacher has a stronger effect than base resolution training. (2) We also try adding a second discriminator so that one focuses entirely on the global low-resolution image, and the other entirely on patches. Both discriminators are initialized with the result from pretraining, but we find that this setting leads to suboptimal metrics, compared to using a single discriminator. (3) We inject scale information into the discriminator following a similar method as the generator via weight modulation. In this case, the training becomes unstable as the discriminator is able to out-compete the generator. 

\myparagraph{Removing the pretraining step.} \lucy{Our final model is first pretrained at a fixed, smaller resolution before varied-size patch training is enabled. This pretraining phase encourages global coherence and also serves as the teacher model later during patch-based training. We conduct an experiment in which the initial pretraining step is omitted, and the model is trained on randomly sampled patches from the start of training. When trained with the same number of HR image patches, the model without global pretraining suffers in both structure and texture -- FID for 1024px generated images is 26.78 and pFID is 8.64 -- compared to our original model which performs global pretraining at low resolution -- FID at 1024px is 4.50 and pFID is 3.46 after 10M training images.}

\subsection{Detectability}

\begin{wrapfigure}{r}{0.5\textwidth}
    \vspace{-12mm}
  \begin{center}
        \includegraphics[width=0.45\textwidth]{figures/CR_forensics.pdf}
  \end{center}
  \vspace{-6mm}
    \caption{\small Detection score from~\cite{wang2020cnn} on our Birds and Mountains datasets. All scores are above chance of $50\%$. Note in both cases, the detectability of our network trends upwards with resolution.\label{fig:detectability}}
  \vspace{-10mm}
\end{wrapfigure}


A concern with improved image generation is the potential for more convincing deceiving images, particularly those of higher resolution, which is the focus of our work.
We use the off-the-shelf detector from Wang et al.~\cite{wang2020cnn} on our Birds (generated $256\rightarrow 2048$) and Mountains ($1024\rightarrow 4096$) generators, across a large range of resolutions. As shown in Figure~\ref{fig:detectability}, the scores are well above chance ($50\%$) across both datasets and resolutions. Interestingly, the curve generally trends upwards, indicating that while higher resolution images may look more natural, they are also easier to detect.


==> sections/sm_03_method.tex <==
\section{Additional implementation details}\label{sec:sm_method}

Building off the StyleGAN3~\cite{karras2021alias} architecture, we describe our coordinate conditioning and scale modulation branch applied to enable generation of multi-scale patches during the second training phase.



\subsection{Patch-based training}

\myparagraph{Extracting patches from varied size images} From our dataset of images \Dataset, we sample
an image $x_i\in \mathds{R}^{H_i\times W_i\times 3} \sim
\Dataset$, with short-side $\NativeResolution=\min(H_i,W_i)$, and take an \NativeResolution-by-\NativeResolution
square crop. We then Lanczos downsample the image to an intermediate resolution $\FullImageResolution \in [\PatchResolution, \NativeResolution]$, which provides ``free'' additional views from the same image, without
introducing image corruptions. 

Next, we sample a random crop of size
\PatchResolution and record the sampling location $v\in \mathds{R}^2$.
To summarize this procedure, we obtain a patch $\ImageSample\in
\mathds{R}^{\PatchResolution \times \PatchResolution \times 3}$ from these two
operations, while saving the sampled image resolution \FullImageResolution and patch center location
$\PatchLocation=(\PatchLocationX, \PatchLocationY)\in [0, 1]^2$ for later use.
\begin{equation}
\ImageSample, \FullImageResolution, \PatchLocation = \mathrm{Crop} ( \mathrm{Downsample} (x_{i}))
\end{equation}

\myparagraph{Synthesizing patches from the generator} Given a set of patches from the image dataset, the generator is tasked with synthesizing images at the corresponding patch locations. To transform the normalized coordinate domain \ContinuousDomain into patch coordinates, we apply a transformation matrix to each 2D location \NormalizedCoordinates in homogenous coordinates:
\begin{equation}
 \Coordinates =  \TransformPatch * \NormalizedCoordinates = 
 \begin{bmatrix}
\frac{\PatchResolution}{\FullImageResolution} & 0 & \PatchLocationX \\
0 & \frac{\PatchResolution}{\FullImageResolution} & \PatchLocationY \\
0 & 0 & 1 \\
\end{bmatrix}
* \NormalizedCoordinates
\end{equation}

Following StyleGAN3, these transformed coordinates are then encoded as
$K$ random Fourier channels by multiplying by frequencies $B\in \mathds{R}^{K
\times 2}$ and adding phases $\phi\in \mathds{R}^{K}$.
For patch synthesis, the Fourier feature extraction at index $(h,w)$ becomes:
\begin{equation}
F_{h,w}(\Coordinates)=\sin \big(2\pi \hspace{.5mm} B \Coordinates + \phi \big) \in \mathds{R}^{K},
\end{equation}


\subsection{Scale-conditioning branch}

As individual coordinate positions \Coordinates do not directly convey scale information, we found it beneficial additionally incorporate the scale input to intermediate layers of the generator. To do this, we first normalize the target scale \FullImageResolution to $[0, 1]$ using:
\begin{equation}
    \NormalizedFullImageResolution = \frac{\FullImageResolution - \PatchResolution}{\MaxNormImageResolution - \PatchResolution} 
\end{equation}
where \MaxNormImageResolution is selected from dataset statistics and is only present as a normalization factor, but does not clip the upper synthesis bound during inference. \lucy{Empirically, we found that adding a small offset factor (we use $0.1$) to the normalized target scale \NormalizedFullImageResolution allows for smoother interpolations between resolutions by avoiding a discontinuity at zero.}

We then encode \NormalizedFullImageResolution using a parallel mapping network of identical architecture to the latent mapping network $\AuxNetwork(\LatentCode)$, and add the two inputs after undergoing a layer-specific affine transformation into style-space~\cite{wu2021stylespace,patashnik2021styleclip} to obtain the final modulation parameter $\AuxNetwork(\LatentCode, \FullImageResolution)_k$ at layer $k$:
\begin{equation}
   \AuxNetwork(\LatentCode, \FullImageResolution)_k = (W_{z, k} * \AuxNetwork_z(\LatentCode) + b_{z, k}) +  (W_{s, k} * \AuxNetwork_s(\FullImageResolution) + b_{s, k})
\end{equation}
Because the modulation parameter is a multiplicative factor on the network weights and the scale-conditioning portion is added only during the secondary patch-wise training step, we initialize $b_{z, k} = \mathbf{1}$ and $b_{s, k} = \mathbf{0}$ to allow the network to smoothly transition between the initial pretraining step and secondary patch-based training. 





\subsection{Training procedure}

We train our models on four to eight V100 GPUs
with 16GB memory.
By sampling fixed-size patches, the memory and compute
footprint remain constant during training.
For FFHQ, we finetune our initial fixed-scale generator from the pretrained
FFHQ-U model~\cite{karras2021alias}, which reaches a minimum FID within 4M
training images.
In the remaining domains, we perform the pretraining step
from scratch, retaining the checkpoint with the lowest
FID, computed over 25M image samples, before
continuing with the second, mixed-resolution training phase.
Our training procedure is compatible with both 3$\times$3 and 1$\times$1 kernel
sizes in StyleGAN3 (T \& R configurations, respectively). For the patch-based training step, we proceed with the model configuration that reaches the best FID in pretraining, which is typically Config T with the exception of the FFHQ domain.



